Small Vision-Language Models are Smart Compressors for Long Video Understanding

Adapting Multimodal Large Language Models (MLLMs) for hour-long videos is bottlenecked by context limits. Dense visual streams saturate token budgets and exacerbate the lost-in-the-middle phenomenon. Existing heuristics, like sparse sampling or uniform pooling, blindly sacrifice fidelity by discarding decisive moments and wasting bandwidth on irrelevant backgrounds. We propose Tempo, an efficient query-aware framework compressing long videos for downstream understanding. Tempo leverages a Small Vision-Language Model (SVLM) as a local temporal compressor, casting token reduction as an early cross-modal distillation process to generate compact, intent-aligned representations in a single forward pass. To enforce strict budgets without breaking causality, we introduce Adaptive Token Allocation (ATA). Exploiting the SVLM's zero-shot relevance prior and semantic front-loading, ATA acts as a training-free $O(1)$ dynamic router. It allocates dense bandwidth to query-critical segments while compressing redundancies into minimal temporal anchors to maintain the global storyline. Extensive experiments show our 6B architecture achieves state-of-the-art performance with aggressive dynamic compression (0.5-16 tokens/frame). On the extreme-long LVBench (4101s), Tempo scores 52.3 under a strict 8K visual budget, outperforming GPT-4o and Gemini 1.5 Pro. Scaling to 2048 frames reaches 53.7. Crucially, Tempo compresses hour-long videos substantially below theoretical limits, proving true long-form video understanding relies on intent-driven efficiency rather than greedily padded context windows.

==> eq/adaptive_linear_budget_allocation.tex <==
\begin{equation}
    k_i^{ideal} = k_{min} + \lfloor \hat{s}_i \cdot (k_{max} - k_{min}) \rfloor
  \label{eq:linear_allocation}
\end{equation}

==> eq/adaptive_soft_budget_allocation.tex <==
\begin{equation}
    k_i = k_{min} + \lfloor w_i \cdot B_{res} \rfloor, \quad \text{where} \quad w_i = \frac{\hat{s}_i}{\sum_{j=1}^N \hat{s}_j}
  \label{eq:soft_allocation}
\end{equation}

==> eq/loss.tex <==
\begin{equation}
    \mathcal{L}_{\mathrm{AR}}(\theta,\phi) = -\sum_{t=1}^{T}\log p_{\theta}\big(a_t \mid a_{<t}, Q, \{\tilde{\mathbf{H}}_i\}_{i=1}^{N}\big)
    \label{eq:loss}
\end{equation}

==> eq/relevance.tex <==
\begin{equation}
    s_i = \sigma \left( \mathbf{w}_{yes}^\top \mathbf{h}_{prev} - \mathbf{w}_{no}^\top \mathbf{h}_{prev} \right)
    \label{eq:relevance}
\end{equation}

==> image.tex <==

\begin{figure*}[t]
     \centering
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[]{assets/plot_demo.pdf}
         \caption{First plot.}
         \label{fig:plots:a}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[]{assets/plot_demo.pdf}
         \caption{Second plot.}
         \label{fig:plots:b}
     \end{subfigure}
     \caption{Plots generated with the script \texttt{nice\_plot.py} included in this template.
     % 
     For more information on producing figures, please refer to \href{https://fb.workplace.com/notes/1767028093764250}{this Workplace post}.
     %
     If you would like to use a figure teaser, place it immediately after \texttt{\textbackslash{}maketitle}, forcing its location with the \texttt{[h!]} optional argument.
     %
     Please consider using the \href{https://www.facebook.com/brand/meta/color/}{Meta palette} to color your figures.
     }
     \label{fig:plots}
\end{figure*}

==> table.tex <==

\begin{table*}[t]
    \centering
    \begin{NiceTabular}{lcccccc}
    \CodeBefore
    \rectanglecolor{metabg}{3-4}{4-4}
    \rectanglecolor{metabg}{5-6}{6-6}
    \Body
    \toprule
                               &   & \multicolumn{3}{c}{Vision tasks} & \multicolumn{2}{c}{Language tasks}\\
    \cmidrule{3-7}
                               &               & DatasetA             & DatasetB             & DatasetC             & DatasetD             & DatasetE \\
    \midrule
    \multirow{2}{*}{BaselineA} & $\lambda = 0$ & $\nm{0.84 \pm 0.22}$ & $\bm{0.83 \pm 0.14}$ & $\nm{0.84 \pm 0.24}$ & $\nm{0.86 \pm 0.16}$ & $\nm{0.81 \pm 0.18}$\\
                               & $\lambda = 1$ & $\nm{0.83 \pm 0.26}$ & $\nm{0.82 \pm 0.20}$ & $\nm{0.88 \pm 0.23}$ & $\nm{0.87 \pm 0.12}$ & $\nm{0.84 \pm 0.20}$\\
    \multirow{2}{*}{BaselineB} & $\lambda = 0$ & $\nm{0.84 \pm 0.15}$ & $\nm{0.86 \pm 0.16}$ & $\nm{0.89 \pm 0.11}$ & $\nm{0.84 \pm 0.17}$ & $\nm{0.87 \pm 0.30}$\\
                               & $\lambda = 1$ & $\bm{0.90 \pm 0.15}$ & $\nm{0.81 \pm 0.22}$ & $\nm{0.88 \pm 0.18}$ & $\nm{0.83 \pm 0.23}$ & $\nm{0.80 \pm 0.27}$\\
    \midrule 
    \textbf{Our method}        &               & $\nm{0.86 \pm 0.19}$ & $\nm{0.81 \pm 0.18}$ & $\bm{0.95 \pm 0.16}$ & $\bm{0.91 \pm 0.13}$ & $\bm{0.92 \pm 0.30}$\\
    \bottomrule
    \end{NiceTabular}
    \caption{A nice table does not require vertical separators and uses bolding---here implemented by the \texttt{\textbackslash{}bm\{\}} and \texttt{\textbackslash{}nm\{\}} commands---sparingly.
    %
    Using the \texttt{NiceTabular} environment from the \texttt{nicematrix} package to highlight the background of some cells easily, using the official \texttt{metabg} color.}
    \label{table:demo}
\end{table*}
